Unsupervised Representation Learning by Sorting Sequences

We present an unsupervised representation learning approach using videos without semantic labels. We leverage the temporal coherence as a supervisory signal by formulating representation learning as a sequence sorting task. We take temporally shuffled frames (i.e., in non-chronological order) as inputs and train a convolutional neural network to sort the shuffled sequences. Similar to comparison-based sorting algorithms, we propose to extract features from all frame pairs and aggregate them to predict the correct order. As sorting shuffled image sequence requires an understanding of the statistical temporal structure of images, training with such a proxy task allows us to learn rich and generalizable visual representation. We validate the effectiveness of the learned representation using our method as pre-training on high-level recognition problems. The experimental results show that our method compares favorably against state-of-the-art methods on action recognition, image classification and object detection tasks.

==> table_related.tex <==
\begin{table}[t]
	\caption{Summary of different unsupervised method, upper part of table lists image-based methods, lower part of table lists video-based methods.}
	\label{tab:related}
	\vspace{1mm}
	\centering
	\small
	
	\begin{tabular}{cc}
		\hline 
		Method  & Task \\
		\hline
		Doerch \etal \cite{doersch2015context} & prediction relative patch location \\
		Pathak \etal \cite{pathak2016inpainting}  & image inpainting  \\
		Norrozi \etal \cite{noroozi2016puzzle}  & patche puzzle solving \\ 
		Zhang \etal \cite{zhang2016splitbrain}  & cross-channel reconstruction \\
		Larsson \etal \cite{larsson2016colorization}  & colorization \\ 
		Zhang \etal \cite{zhang2016colorization2}  &　colorization \\
		Isola \etal \cite{isola2015cooccur}  & co-occurrence \\ 
		Owens \etal \cite{owens2016ambient}  & sounds \\ 
		\hline
		Wang and Gupta\cite{wang2015unsupervised}  & object variance via tracking \\
		Jayaraman \etal \cite{jayaraman2015slowandsteady}  & temporal coherence \\
		Agrawal \etal \cite {agrawal2015ego}& transformation in ego-motion \\
		Jayaraman \etal \cite{jayaraman2015ego} & transformation in ego-motion \\
		Misra \etal \cite{misra2016shuffle}  & sequence order correctness \\
		Purushwalkam and Gupta \cite{purushwalkam2016transformation} & optical flows as transformation \\
		TR (ours)  & rearrange shuffled sequence\\
	\end{tabular}
	
	\vspace{-2mm}
\end{table}
